Caching and Reproducibility: Making Data Science experiments faster and FAIRer

Small to medium-scale data science experiments often rely on research software developed ad-hoc by individual scientists or small teams. Often there is no time to make the research software fast, reusable, and open access. The consequence is twofold. First, subsequent researchers must spend significant work hours building upon the proposed hypotheses or experimental framework. In the worst case, others cannot reproduce the experiment and reuse the findings for subsequent research. Second, suppose the ad-hoc research software fails during often long-running computationally expensive experiments. In that case, the overall effort to iteratively improve the software and rerun the experiments creates significant time pressure on the researchers. We suggest making caching an integral part of the research software development process, even before the first line of code is written. This article outlines caching recommendations for developing research software in data science projects. Our recommendations provide a perspective to circumvent common problems such as propriety dependence, speed, etc. At the same time, caching contributes to the reproducibility of experiments in the open science workflow. Concerning the four guiding principles, i.e., Findability, Accessibility, Interoperability, and Reusability (FAIR), we foresee that including the proposed recommendation in a research software development will make the data related to that software FAIRer for both machines and humans. We exhibit the usefulness of some of the proposed recommendations on our recently completed research software project in mathematical information retrieval.

==> manuscript_contributions.tex <==
In Data Science, research software is important for performing experiments and proving hypotheses. After the initial hypothesis, a first prototype is developed and modified in further steps until the desired result is produced. Thereafter the results are published as fast as possible in order to claim the scientific achievement. Overall development technique puts high pressure on the developers of the research software. This procedure is problematic for various reasons: 1) The modifications of the software lead to a significant performance decrease and researchers have to spend a significant time waiting for results of intermediate runs. 2) When runs of the research software fail under seldom conditions in the input data, it is often not possible to continue with an improved version of the software from the position in the dataset where the last version ended. 3) Even if software and datasets are provided, the original reported results can often not be reproduced due to external dependencies or commercial software that cant be published. We provide a perspective for caching data science experiments to improve upon some of these problems. We propose a general set of guidelines suitable for developing any research software, which contributes to the goal of reproducibility.


